Introduction to OXPath

Contemporary web pages with increasingly sophisticated interfaces rival traditional desktop applications for interface complexity and are often called web applications or RIA (Rich Internet Applications). They often require the execution of JavaScript in a web browser and can call AJAX requests to dynamically generate the content, reacting to user interaction. From the automatic data acquisition point of view, thus, it is essential to be able to correctly render web pages and mimic user actions to obtain relevant data from the web page content. Briefly, to obtain data through existing Web interfaces and transform it into structured form, contemporary wrappers should be able to: 1) interact with sophisticated interfaces of web applications; 2) precisely acquire relevant data; 3) scale with the number of crawled web pages or states of web application; 4) have an embeddable programming API for integration with existing web technologies. OXPath is a state-of-the-art technology, which is compliant with these requirements and demonstrated its efficiency in comprehensive experiments. OXPath integrates Firefox for correct rendering of web pages and extends XPath 1.0 for the DOM node selection, interaction, and extraction. It provides means for converting extracted data into different formats, such as XML, JSON, CSV, and saving data into relational databases. This tutorial explains main features of the OXPath language and the setup of a suitable working environment. The guidelines for using OXPath are provided in the form of prototypical examples.

==> tables/oxpath/functions.tex <==
\begin{longtable}{l X}
  \caption{OXPath-specific functions}\label{oxpath:t:functions} \\
  \toprule\textbf{Function} & \textbf{Description} \\ \toprule\endfirsthead
  \toprule\textbf{Function} & \textbf{Description} \\ \toprule\endhead
  to-xml() & Return a string serialization of the XML representation of the current element \\ \nopagebreak\midrule
  is-visible() & Returns \texttt{true} if current element has been visualized by the web browser and has non-empty area\\ \nopagebreak\midrule
  qualify-url() & Return the URL relative to the URL of a current web page \\ \nopagebreak\midrule
%TODO check the correctness of select-text() !
%  select-text() & Highlight the specified set of elements \\ \nopagebreak\midrule
  dom-property() & Return the property of the current DOM node. For example, \texttt{dom-property("nodeType")} returns the type of a DOM node. \\ \nopagebreak\midrule
  innerhtml() & Return the \texttt{innerHTML} property of a current node.\\ \nopagebreak\midrule
  outerhtml() & Return the \texttt{outerHTML} property of a current node. \\ \nopagebreak\midrule
%TODO: This function is not supported
%  save-page() & ??? \\ \nopagebreak\midrule
  jaro-wrinkler() & Return the similarity between two arguments (DOM nodes or strings) in terms of Jaro-Winkler distance. The value is in the range from 0 to 1, the higher the similarity the higher the value. Two arguments are required.\\ \nopagebreak\midrule
  page-content() & Return a string serialization of HTML of a current state of a web page. It does not require any arguments. \\ \nopagebreak\midrule
  current-url() & Return the URL of a current web page. It does not require any arguments.\\ \nopagebreak\midrule
  now() & Create a timestamp in a form \texttt{yyyy-MM-dd'T'HH:mm:ss'Z'}. It does not require any arguments.\\ \nopagebreak\midrule
  %This is commented deliberatly.
%  urify() & Return the part of the URI after the last \texttt{/}, all substrings of symbols which are not \texttt{\\W}, are replaced by \texttt{_}. \\ \nopagebreak\midrule
  screenshot() & Load a web page with the URL of a current web page into a new window and makes a screenshot. It returns the path to the file created. The path has the following form \texttt{\textit{host\_timestamp}}, in which all characters of \texttt{\textit{host\_timestamp}} matching the regular expression ``\texttt{\textbackslash{}W}'' are replaced by ``\texttt{\_}'', \texttt{\textit{timestamp}} has the format ``\texttt{ddMMM\_HHmmss}''. \\ \nopagebreak\midrule
%  position() & get position number of current node in current result sequence \\ \nopagebreak\midrule
%  last() & get position number of last node in current result sequence \\ \nopagebreak\midrule
%  count() & count number of nodes in current result set \\ \nopagebreak\midrule
%TODO this is not implemented! Use #= instead!
%  id() & select element with specific id \\ \nopagebreak\midrule
%  namespace-uri() & get namespace of an element \\ \nopagebreak\midrule
%  local-name() & get local name of a node set \\ \nopagebreak\midrule
%  name() & get name of a node set \\ \nopagebreak\midrule
%  string() & convert argument to string \\ \nopagebreak\midrule
  string-join() & Join textual content of DOM nodes. The first argument is a node set, the second is a string (a separator).
  The third argument is optional and specifies the procedure for obtaining the textual representation of nodes. The following values are accepted: ``to-xml'', ``normalize-space'', ``innerhtml'', and ``outerhtml''. \\ \nopagebreak\midrule
%  concat() & concatenate string arguments \\ \nopagebreak\midrule
%  starts-with() & check string for specific prefix \\ \nopagebreak\midrule
%  contains() & check for specific substring \\ \nopagebreak\midrule
%
  opex:minus() & Subtract the second argument from the first one. \\ \nopagebreak\midrule
  opex:plus() & Add the first and the second arguments. \\ \nopagebreak\midrule
%
  substring-before() & Get a substring (a string) that is the rest of the string representing the first argument (a DOM node) before a substring given by the second parameter.
  For example, \texttt{substring-before(., "separator")}.
  The third parameter is optional and specifies the ordinal number of the occurrence of the second argument to be considered as a separator.
  (It is 1 by default.)
  For example, \texttt{substring-before(., "separator", 5)} returns the substring of the first argument that starts from the beginning of the string and ends just before the 5th occurrence of the substring ``separator''. \\ \nopagebreak\midrule
%
  substring-after() & Get a substring (a string) that is the rest of the string representing the first argument (a DOM node) after a substring given by the second parameter.
  For example, \texttt{substring-after(., "separator")}.
  The third parameter is optional and specifies the ordinal number of the occurrence of the second argument to be considered as a separator.
  (It is 1 by default.)
  For example, \texttt{substring-after(., "separator", 5)} returns the substring of the first argument that starts just after the 5th occurrence of the substring ``separator'' and ends at the end of the string. \\ \nopagebreak\midrule
%
  substring-before-reverse() & Return a substring as in \texttt{substring-before}, but, in contrast, the search of the ``separator'' is conducted in a reverse direction, i.e., from the last to the first character of the string. \\ \nopagebreak\midrule
%
  substring-after-reverse() & Return a substring as in \texttt{substring-after}, but, in contrast, the search of the ``separator'' is conducted in a reverse direction, i.e., from the last to the first character of the string. \\ \nopagebreak\midrule
%
  substring-reverse() & Returns a substring as XPath's \texttt{substring} function, but, in contrast, the input string is reverted. \\ \nopagebreak\bottomrule
%
%  string-length() & count number of chars in a string \\ \nopagebreak\midrule
%  normalize-space() & trim whitespace of string argument \\ \nopagebreak\midrule
%  translate() & ??? \\ \nopagebreak\midrule
%  replace() & replace elements in a string, e.g. with regular expressions \\ \nopagebreak\midrule
%  matches() & check if string argument matches specified regular expression \\ \nopagebreak\midrule
%  boolean() & evaluate argument to true or false \\ \nopagebreak\midrule
%  not() & negate argument \\ \nopagebreak\midrule
%  true() & create boolean value of \texttt{false} \\ \nopagebreak\midrule
%  false() & create boolean value of \texttt{true} \\ \nopagebreak\midrule
%  lang() & compare language code of element with specified language code \\ \nopagebreak\midrule
%  number() & convert argument to a number \\ \nopagebreak\midrule
%  sum() & add up numeric arguments \\ \nopagebreak\midrule
%  floor() & round down numeric argument \\ \nopagebreak\midrule
%  ceiling() & round up numeric argument \\ \nopagebreak\midrule
%  round() & round a number \\ \nopagebreak\bottomrule
\end{longtable}

% \nopagebreak


==> tables/xpath/w3s_predicates.tex <==
\begin{longtable}{l X}
  \caption{W3Schools examples of XPath predicates}\label{xpath:t:predicates} \\
  \toprule\textbf{Path Expression} & \textbf{Result} \\ \toprule\endfirsthead
  \toprule\textbf{Path Expression} & \textbf{Result} \\ \toprule\endhead
  /bookstore/book[1] & First book element \\ \nopagebreak\midrule
  /bookstore/book[last()] & Last book element \\ \nopagebreak\midrule
  /bookstore/book[last()-1] & Last but one book element \\ \nopagebreak\midrule
  /bookstore/book[position()$<$3] & First two book elements \\ \nopagebreak\midrule
  //*[@lang] & Any element with @lang \\ \nopagebreak\midrule
  //*[@lang='en'] & Any element with @lang="en" \\ \nopagebreak\midrule
  /bookstore/book[price$>$35.00]/title & further step after predicate \\
  \bottomrule
\end{longtable}


==> users/chapters/include/oxpathInAction/cambridge.tex <==
%------------------------------------------------------------------------------
\subsection{Example: Journal of Functional Programming}\label{oia:extract:cambridge}
%------------------------------------------------------------------------------

\begin{figure}[h]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/cambridge-robotica-loi-00.png}
	\caption{Homepage of the journal \emph{Robotica} at Cambridge Core\label{oia:toc:fig:cambridge:robotica:loi:00}}
\end{figure}

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/cambridge-robotica-loi-01.png}
  	\caption{List of all issues for the journal \emph{Robotica}\label{oia:toc:fig:cambridge:robotica:loi:01}}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/cambridge-robotica-loi-02.png}
    \caption{List of all issues for the journal \emph{Robotica}\label{oia:toc:fig:cambridge:robotica:loi:02}}
  \end{minipage}
\end{figure}

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/cambridge-robotica-loi-03.png}
  	\caption{List of all issues for the journal \emph{Robotica}\label{oia:toc:fig:cambridge:robotica:loi:03}}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/cambridge-robotica-loi-04.png}
    \caption{Volume 26 of the journal \emph{Robotica}\label{oia:toc:fig:cambridge:robotica:loi:04}}
  \end{minipage}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/cambridge-robotica-toc-00.png}
	\caption{Table of contents for \emph{Robotica} Volume 34, Issue 12\label{oia:toc:fig:cambridge:robotica:toc:00}}
\end{figure}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=oxpath,
    caption={OXPath expression for the list of issues of \emph{Robotica}\label{oia:toc:oxp:cambridge:robotica:loi:00}}
  ]{users/chapters/listings/oxpathInAction/oxp/cambridge-robotica-loi.aoxp}
\end{minipage}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=oxpath,
    caption={OXPath expression for the table of contents of \emph{Robotica} Volume 34, Issue 12\label{oia:toc:oxp:cambridge:robotica:toc:00}}
  ]{users/chapters/listings/oxpathInAction/oxp/cambridge-robotica-toc.aoxp}
\end{minipage}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=xml,
    caption={XML output for the list of issues of \emph{Robotica}\label{oia:toc:xml:cambridge:robotica:loi:00}}
  ]{users/chapters/listings/oxpathInAction/xml/cambridge-robotica-loi.axml}
\end{minipage}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=xml,
    caption={XML output for the table of contents of \emph{Robotica} Volume 34, Issue 12\label{oia:toc:xml:cambridge:robotica:toc:00}}
  ]{users/chapters/listings/oxpathInAction/xml/cambridge-robotica-toc.axml}
\end{minipage}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=html,
    caption={HTML source for the table of contents of \emph{Robotica} Volume 34, Issue 12\label{oia:toc:html:cambridge:robotica:toc:00}}
  ]{users/chapters/listings/oxpathInAction/html/cambridge-robotica-toc.ahtml}
\end{minipage}


==> users/chapters/include/oxpathInAction/edm.tex <==
%------------------------------------------------------------------------------
\subsection{Example: Educational Data Mining}\label{oia:toc:edm}
%------------------------------------------------------------------------------


The proceedings of conferences often can be found in the form of tables of content on the homepages of the responsible societies. For example, the International Educational Data Mining Society (IEDMS) publishes the proceedings of the International Conference on Educational Data Mining (EDM) on their homepage (Figure \ref{oia:toc:fig:edm:00}). The following OXPath example extracts the table of contents of the 2014 EDM proceedings.

\begin{figure}[h]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/edm-00.png}
	\caption{International Educational Data Mining Society\label{oia:toc:fig:edm:00}}
\end{figure}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=oxpath,
    caption={OXPath expression for the EDM 2014 Proceedings\label{oia:toc:oxp:edm2014:00}}
  ]{users/chapters/listings/oxpathInAction/oxp/edm2014-a-00.aoxp}
\end{minipage}

The following steps briefly summarise the necessary steps for this this task: (\textbf{1}) Visit the website of IEDMS. (\textbf{2}) Navigate to the homepage of EDM 2014. (\textbf{3}) Continue to the proceedings page of the conference. (\textbf{4}) Identify the individual publications. (\textbf{5}) Retrieve details for each publication.

The expression in Listing \ref{oia:toc:oxp:edm2014:00} constitutes the same list of steps in OXPath syntax. The call of the \texttt{doc()}-function in line 1 fulfils step (\textbf{1}). Line 2 navigates to the section for sponsored events on the IEDMS homepage to select and click the link to the EDM 2014 homepage (s. Figure \ref{oia:toc:fig:edm:01}), constituting step (\textbf{2}). For step (\textbf{3}), the following line of the OXPath expression selects the menu entry containing the string \enquote{Proceedings} from the navigation bar on the left in Figure \ref{oia:toc:fig:edm:2014:02}. Finally, line 4 identifies the individual publications such as the one highlighted in Figure \ref{oia:toc:fig:edm:2014:03} (\textbf{4}).

\begin{figure}[h]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/edm-01.png}
	\caption{Navigating to Educational Data Mining 2014\label{oia:toc:fig:edm:01}}
\end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.48\textwidth}
%     \centering
%   	\includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/edm2014-02.png}
%   	\caption{Navigating to the Proceedings of Educational Data Mining 2014\label{oia:toc:fig:edm:2014:02}}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.48\textwidth}
%     \centering
%   	\includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/edm2014-03.png}
%   	\caption{Identifying the publications of EDM 2014\label{oia:toc:fig:edm:2014:03}}
%   \end{minipage}
% \end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/edm2014-02.png}
	\caption{Navigating to the Proceedings of Educational Data Mining 2014\label{oia:toc:fig:edm:2014:02}}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/edm2014-03.png}
	\caption{Identifying the publications of EDM 2014\label{oia:toc:fig:edm:2014:03}}
\end{figure}

The remaining lines of the OXPath expression deal with the extraction of the metadata fields for each publication (\textbf{5}). EDM 2014 is an example of a table of content that does not distinguish the individual fields with element classes. Listing \ref{oia:toc:html:edm2014:00} shows an excerpt of the HTML source code of the EDM 2014 proceedings website to explain the location paths in lines 4-9 of Listing \ref{oia:toc:oxp:edm2014:00}.

The individual publications are contained in \texttt{<p>} elements which also contain an \texttt{<em>} element. For each of these elements a \texttt{record} element is extracted. The content of this \texttt{<em>} element constitutes the author list of each record and is extracted as an \texttt{authors} element for each \texttt{record} in line 5. The first text-node child inside each relevant \texttt{<p>} node is extracted as the \texttt{title} of each \texttt{record}. To extract the page-range information (\texttt{pages}), line 7 retrieves the first text-node sibling following the second line break. The \texttt{url} for the PDF file associated with a \texttt{record} is extracted from the only \texttt{<a>} child of each \texttt{<p>} element. Lastly, line 9 identifies thhe first preceding \texttt{<strong>} element and extracts its contents as the section \texttt{header} of the current record.

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=xml,
    caption={XML output of the EDM 2014 Proceedings\label{oia:toc:xml:edm2014:00}}
  ]{users/chapters/listings/oxpathInAction/xml/edm2014-a-00.axml}
\end{minipage}

With the help of XPath functions the OXPath expression in Figure \ref{oia:toc:oxp:edm2014:00} and its output in Figure \ref{oia:toc:xml:edm2014:00} can be refined. Unwanted leading or trailing whitespace such as in the author list in line 5 in Figure \ref{oia:toc:xml:edm2014:00} can be eliminated with \texttt{normalize-space()}. Furthermore, the page range information can be extracted more precisely with the help of \texttt{replace()} and regular expressions. The relative URI to the PDF file of a record can also be made absolute with the help of \texttt{concat()}. The new expression and its output are shown in Figures \ref{oia:toc:oxp:edm2014:01} and \ref{oia:toc:xml:edm2014:01}.

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=oxpath,
    caption={Adapted OXPath expression for the EDM 2014 Proceedings\label{oia:toc:oxp:edm2014:01}}
  ]{users/chapters/listings/oxpathInAction/oxp/edm2014-b-00.aoxp}
\end{minipage}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=xml,
    caption={Adapted XML output of the EDM 2014 Proceedings\label{oia:toc:xml:edm2014:01}}
  ]{users/chapters/listings/oxpathInAction/xml/edm2014-b-00.axml}
\end{minipage}

TODO:

\begin{itemize}
  \item hint at order here?
  \item hint at preceding turning order vice versa in XPath
  \item continue with adaptation to EDM 2016
\end{itemize}

\begin{minipage}{\textwidth}
  \lstinputlisting[%
    language=html,
    caption={HTML source of the EDM 2014 Proceedings\label{oia:toc:html:edm2014:00}}
  ]{users/chapters/listings/oxpathInAction/html/edm2014-00.ahtml}
\end{minipage}


==> users/chapters/include/oxpathInAction/ox-ac-comjnl.tex <==
\begin{figure}[!htbp]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/ox-ac-comjnl-loi-1.png}
	\caption{Issue overview for \emph{The Computer Journal} on Oxford Academic\label{fig:oia:start:ox:ac:comjnl:loi:1}}
\end{figure}

Oxford University Press publishes journals via its online content delivery platform Oxford Academic.
The overview page for the list of issues of an individual journal, such as \emph{The Computer Journal}, primarily shows the table of contents for the most recent issue.
Retrieving the list of all available issues and retrieving the individual publications of a specific issue constitute the two main tasks in the following examples.

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/ox-ac-comjnl-loi-2.png}
  	\caption{Accessing the list of all issues for \emph{The Computer Journal}\label{fig:oia:start:ox:ac:comjnl:loi:2}}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=7.5cm]{users/chapters/graphics/oxpathInAction/ox-ac-comjnl-loi-all.png}
    \caption{List of publication years for \emph{The Computer Journal}\label{fig:oia:start:ox:ac:comjnl:loi:all}}
  \end{minipage}
\end{figure}

One option of retrieving the list of issues for \emph{The Computer Journal} is illustrated in Figure \ref{fig:oia:start:ox:ac:comjnl:loi:1} (p. \pageref{fig:oia:start:ox:ac:comjnl:loi:1}). By subsequently selecting the years available in the first drop-down menu \enquote{Select Year}, the second drop-down list contains all issues published in the selected year. However, an OXPath expression clicking through these drop-down items would cause the website to load the table of content for the issue published first in each year. Therefore, a less load-intensive option on the bottom of the issue-overview page is pursued first.

\begin{figure}[!htbp]
	\centering
	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/ox-ac-comjnl-loi-1.png}
	\caption{List of issues for \emph{The Computer Journal}, Volume XX\label{fig:oia:start:ox:ac:comjnl:loi:one}}
\end{figure}

Following the link labelled \enquote{All issues} at the bottom of the issue-overview page (s. Figure \ref{fig:oia:start:ox:ac:comjnl:loi:2}, p. \pageref{fig:oia:start:ox:ac:comjnl:loi:2}) leads to a list of publication years for \emph{The Computer Journal} (s. Figure \ref{fig:oia:start:ox:ac:comjnl:loi:all}, p. \pageref{fig:oia:start:ox:ac:comjnl:loi:all}). Each listed year is actually a link to a list of all the issues published in that year. Each listed issue is represented by a link to the table of contents for that issue. The following OXPath expressions clicks each link for a listed year and collects the available information for the issues of that year. The expression in Figure \ref{oxp:oia:start:ox:ac:comjnl:loi:click}%TODO reference not available; also, it should say 'Listing', not 'Figure'
visits the the list-of-years page  the accessed via the URL of the \enquote{All issues} in Figure \ref{fig:oia:start:ox:ac:comjnl:loi:2} (p. \pageref{fig:oia:start:ox:ac:comjnl:loi:2}) and clicks each of the year links.







% The \emph{Association for Computational Linguistics} (ACL) gives a clear overview its events in its digital library, the \emph{ACL Anthology} (s. Figure \ref{fig:oia:start:acl:dl}). The hompage of the ACL Anthology is a collection of links to individual events. These links lead to very simply structured tables of content, such as in Figure \ref{fig:oia:start:acl:conll:16} for the \emph{Proceedings of the 20th SIGNLL Conference on Computational Natural Language Learning} (CoNLL 2016). Individual publications are presented in individual paragraphs ({\color{MaterialOrange}\texttt{p}} elements).
%
% \begin{figure}[!tbp]
% 	\centering
% 	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/acl-conll-16-p.png}
% 	\caption{Proceedings of CoNLL 2016\label{fig:oia:start:acl:conll:16}}
% \end{figure}
%
% As with every OXPath expression, the target web page with the proceedings of CoNLL 2016 is visited via the {\color{MaterialRed}\texttt{doc()}} function. Devising the OXPath expression for the extraction of publication records is based on the DOM tree of the visited page in Listing \ref{html:oia:start:acl:conll:16} below.%(p. \pageref{html:oia:start:acl:conll:16}).
%
% \begin{minipage}{\textwidth}
%   \newcommand*{\CommonPath}{users/chapters/listings/oxpathInAction/html}
%   \lstinputlisting[%
%     language=html,
%     linerange=1-30,
%     caption={HTML source for the web page of CoNLL 2016\label{html:oia:start:acl:conll:16}}
%   ]{\CommonPath/acl-conll-16.ahtml}
% \end{minipage}
%
% For each publication, i.e. each {\color{MaterialOrange}\texttt{p}} element in the unique {\color{MaterialOrange}\texttt{div}} shown in line 2 of Listing \ref{html:oia:start:acl:conll:16}, a {\color{MaterialGreen}\texttt{record}} node is created as a container in the result tree.
%
% \begin{minipage}{\textwidth}
%   \newcommand*{\CommonPath}{users/chapters/listings/oxpathInAction}
%   \lstinputlisting[%
%     language=oxpath,
%     caption={OXPath expression for the proceedings of CoNLL 2016 with respective XML output: record identification and extraction\label{oxp:oia:start:acl:conll:16:1}}
%   ]{\CommonPath/oxp/acl-conll-16-1.aoxp}
%   \lstinputlisting[%
%     language=xml,
%   ]{\CommonPath/xml/acl-conll-16-1.axml}
% \end{minipage}
%
% Inside each {\color{MaterialOrange}\texttt{p}} element (s. Listing \ref{html:oia:start:acl:conll:16}, p. \pageref{html:oia:start:acl:conll:16}, ll. 7--13), several data fields are available in separate subordinate elements. Each {\color{MaterialOrange}\texttt{a}} element provides a link to the PDF file of the publication (l. 8),  the following {\color{MaterialOrange}\texttt{b}} element lists the authors (l. 10), and the {\color{MaterialOrange}\texttt{i}} element contains the publication title (l. 12). By adding location steps with extraction markers to the basic OXPath expression in Listing \ref{oxp:oia:start:acl:conll:16:1} (p. \pageref{oxp:oia:start:acl:conll:16:1}), these data fields can be included for each of the {\color{MaterialGreen}\texttt{record}} containers. In order to create these new output elements as children of the {\color{MaterialGreen}\texttt{record}}-node containers, the respective sub-expressions have to be put in predicate brackets following the {\color{MaterialGreen}\texttt{record}} extraction marker (s. Listing \ref{oxp:oia:start:acl:conll:16:2}, p. \pageref{oxp:oia:start:acl:conll:16:2}, ll. 3-5).
%
% \begin{minipage}{\textwidth}
%   \newcommand*{\CommonPath}{users/chapters/listings/oxpathInAction}
%   \lstinputlisting[%
%     language=oxpath,
%     caption={OXPath expression for the proceedings of CoNLL 2016 with respective XML output: basic data-field extraction\label{oxp:oia:start:acl:conll:16:2}}
%   ]{\CommonPath/oxp/acl-conll-16-2.aoxp}
%   \lstinputlisting[%
%     language=xml,
%   ]{\CommonPath/xml/acl-conll-16-2.axml}
% \end{minipage}
%
% A closer look at the XML output in Listing \ref{oxp:oia:start:acl:conll:16:2} (p. \pageref{oxp:oia:start:acl:conll:16:2}) and the HTML source in Listing \ref{html:oia:start:acl:conll:16} (p. \pageref{html:oia:start:acl:conll:16}) raises the question of refinement options: (1) The URL to the PDF file of a publication is only partially contained in the value of the {\color{MaterialDeepOrange}\texttt{href}} attribute of the {\color{MaterialOrange}\texttt{a}} element. (2) Unnecessary whitespace should be eliminated from the list of authors. (3) The table of content also attributes each publication to a specific section.
%
% These issues can be addressed with the help of (O)XPath functions and an additional predicate for the current form of the OXPath expression. Firstly, the function {\color{MaterialGreen}\texttt{qualify-url()}} in Listing \ref{oxp:oia:start:acl:conll:16:4}, p. \pageref{oxp:oia:start:acl:conll:16:4}, l. 3, completes the partial URL. Secondly, excessive whitespace is removed with the use of {\color{MaterialGreen}\texttt{normalize-space()}} (l. 4). Lastly, the section title can be added to the data fields of each publication record with the help of the axis {\color{MaterialOrange}\texttt{preceding}}, which reverts the order of the sequence of selected {\color{MaterialOrange}\texttt{h1}} nodes, and the numeric predicate {\color{MaterialOrange}\texttt{[1]}} (l. 6), i.e. the second and last {\color{MaterialOrange}\texttt{h1}} node (s. Listing \ref{html:oia:start:acl:conll:16}, p. \pageref{html:oia:start:acl:conll:16}, l. 5) in document order, not the first (l. 3) is selected for the extracted {\color{MaterialGreen}\texttt{record}} in the output example.
%
% \begin{minipage}{\textwidth}
%   \newcommand*{\CommonPath}{users/chapters/listings/oxpathInAction}
%   \lstinputlisting[%
%     language=oxpath,
%     caption={OXPath expression for the proceedings of CoNLL 2016 with respective XML output\label{oxp:oia:start:acl:conll:16:3}}
%   ]{\CommonPath/oxp/acl-conll-16-3.aoxp}
%   \lstinputlisting[%
%     language=xml,
%   ]{\CommonPath/xml/acl-conll-16-3.axml}
% \end{minipage}
%
% \begin{minipage}{\textwidth}
%   \newcommand*{\CommonPath}{users/chapters/listings/oxpathInAction}
%   \lstinputlisting[%
%     language=oxpath,
%     caption={OXPath expression for the proceedings of CoNLL 2016 with respective XML output: refined data-field extraction\label{oxp:oia:start:acl:conll:16:4}}
%   ]{\CommonPath/oxp/acl-conll-16-4.aoxp}
%   \lstinputlisting[%
%     language=xml,
%   ]{\CommonPath/xml/acl-conll-16-4.axml}
% \end{minipage}


==> users/chapters/oxpathInActionMore.tex <==
%------------------------------------------------------------------------------
\clearpage
\section{More OXPath Examples}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\subsection{Extracting from Oxford Academic}\label{oia:start:ox:ac:comjnl}
%------------------------------------------------------------------------------

\input{users/chapters/include/oxpathInAction/ox-ac-comjnl.tex}

%-------------------------------------------------------------------------
\subsection{Books}
%-------------------------------------------------------------------------

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{Cambridge Core}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

The following expression retrieves all books from the subject area of computer science published from \$\{start.year\} to \$\{end.year\} in Cambridge Core.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Cambridge Core Books: Crawl Search and Filter Results]
doc('https://www.cambridge.org/core/browse-subjects/computer-science/listing?sort=canonical.date%3Adesc&aggs%5BproductTypes%5D%5Bfilters%5D=BOOK%2CPUBLISHER_SERIES_COLLECTION')
  //*[@id='startYear']/{"${start.year}" /}
  //*[@id='endYear']/{"${end.year}" }
  /../following-sibling::*/a[contains(., 'Apply')]/{click /}
  /(//hr[1]//following::*[@class='pagination'][1]/li[not(@class='unavailable')]/a[contains(., 'Next')]/{nextclick /})*
  //div[@data-prod-id][.//li[@class="title"]][not(.//*[@class='product-status'][contains(., 'Coming soon')])]:<record>
    [.//li[@class="title"]
      [? ./a[@class="part-link"]
        /.:<title=normalize-space(.)>
        /.:<details=qualify-url(@href)>
      ]
    ]
    [? .//li[@class="author"][1]:<authors=normalize-space(string-join(./a[@class="more-by-this-author"], ', '))>]
    [? .//li[@class="source"]/a:<doi=normalize-space(.)>]
    [? .//li[@class="published"]
      [? .//*[@class="date"]:<date=normalize-space(.)>]
      [? .//following-sibling::*[@class="pages"]:<pages=normalize-space(.)>]
    ]
\end{lstlisting}

The following expression extracts the publication metadata for a given URL to a details page of a book listed by Cambridge Core.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Cambridge Core Book: Publication Metadata]
doc('${url}')
  //*[@id='maincontent']:<record>
    [? ./preceding::section[contains(@class, 'banner')]:<title=string-join(.//h1/text()[normalize-space()] | .//h2/text()[normalize-space()], ': ')>]
    [? .//*[contains(@class, 'main-details')]//li[contains(@class, 'author')][1][contains(., 'Edited by')]
      :<editors=normalize-space(string-join(.//a[ contains(@class, "more-by-this-author")]/span[contains(@class, "author-name")], '; '))>
    ]
    [? .//*[contains(@class, 'main-details')]//li[contains(@class, 'author')][1][not(contains(., 'Edited by'))]
      :<authors=normalize-space(string-join(.//a[ contains(@class, "more-by-this-author")]/span[contains(@class, "author-name")], '; '))>
    ]
    [? .//*[contains(@class, 'main-details')]/following-sibling::div
      [? .//li[./span[1][contains(., 'Publisher:')]]
        :<publisher=normalize-space(./span[2])>
      ]
      [? .//li[./span[1][contains(., 'Online publication date:')]]
        :<date=normalize-space(./span[2])>
      ]
      [? .//li[./span[1][contains(., 'Print publication year:')]]
        :<year=normalize-space(./span[2])>
      ]
      [? .//li[./span[1][contains(., 'Online ISBN:')]]
        :<isbn=normalize-space(./span[2])>
      ]
      [? .//li[./span[1][contains(., 'Book DOI:')]]
        :<doi=normalize-space(./span[2])>
      ]
      [? .:<toc=current-url()>]
      [? .//li[./span[1][contains(., 'Series:')]]
        :<series=replace(normalize-space(./span[2]), "(.*?)\s*?\((\d+)\)", "$1")>/.[contains(., '(')]
        :<volume=replace(normalize-space(./span[2]), "(.*?)\s*?\((\d+)\)", "$2")>
      ]
    ]
\end{lstlisting}

The following expression extracts the table-of-content information for a given URL to a details page of a book listed by Cambridge Core.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Cambridge Core Book: Table of Contents]
doc('${url}')
  /(//hr[1]//following::*[contains(@class, 'pagination')][1]//a[..[not(contains(@class, 'unavailable'))]][contains(., 'Next')]/{click /}
  )*
  //*[starts-with(@class, 'results-listing')]
    //ul[starts-with(@class, 'details')]:<record>
      [? ./..[not(contains(@class, 'indent-0'))]/preceding::*[contains(@class, 'indent-0')][1]//li[contains(@class, 'title')]/a[contains(@class, 'part-link')]/text()[normalize-space()]:<header=normalize-space(.)>]
      [.//li[contains(@class, 'title')]
        [? .:<title=normalize-space(./a[contains(@class, 'part-link')]/text()[normalize-space()])>
        :<pages=normalize-space(.//*[contains(@class, 'pages')])>
        :<details=qualify-url(@href)>
        ]
      ]
      [? .//li[contains(@class, 'author')]
        :<authors=normalize-space(string-join(.//a[ contains(@class, "more-by-this-author")]/span[contains(@class, "author-name")], '; '))>
      ]
      [? .//li[contains(@class, 'source')]
        /a:<doi=normalize-space(.)>
      ]
\end{lstlisting}

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{Computer Science Books by MIT Press}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

The following expression extracts all books from the subject area of computer science dealing with databases and published by the MIT Press.

% TODO: move to correct place
\lstset{
  literate={©}{{\copyright}}1
}

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=AGIT Journal: Table of Contents A]
doc('https://mitpress.mit.edu/cs')
  //*[contains(@class, 'view-discipline-term-list')]//li[contains(., 'Machine Learning and Adaptive Computation')]//a/{click /}
  /(//*[contains(@class, 'pager-top')]//*[contains(@class, 'pager-next')]/a/{click /})*
    //*[@id='sub-discipline']//*[contains(@class, 'view-booklist')]//*[contains(@class, 'views-row')]:<record>
      [? .//*[contains(@class, 'field-title')]
        :<title=normalize-space(.)>]
      [? .//*[contains(@class, 'field-subtitle')]
        :<subtitle=normalize-space(.)>]
      [? .//*[contains(@class, 'field-contributors')][contains(.//span/@itemprop, 'editor')]
        :<editors=string-join(.//span[@itemprop='name'], '; ')>]
      [? .//*[contains(@class, 'field-contributors')][not(contains(.//span/@itemprop, 'editor'))]
        :<authors=string-join(.//span[@itemprop='name'], '; ')>]
      [? .//*[contains(@class, 'field-title')]//a/{click /}
        /.[? .:<details=current-url()>]
          [? .//*[@itemprop='publisher']
            :<publisher=normalize-space(.//*[@itemprop='name']/@content)>]
          [? .//*[@itemprop='dateCreated']
            :<year=substring-before(@content, '-')>]
          [? .//*[@itemprop='isbn']
            :<isbn=normalize-space(.)>]
          [? .:<note=normalize-space(string-join(.//*[contains(@class, 'mitpress-specifications__binding')], '; '))>]
      ]
\end{lstlisting}

%-------------------------------------------------------------------------
\subsection{Theses Archives}
%-------------------------------------------------------------------------

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{ACM Digital Library}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
The following expression extracts all theses listed by the advanced search of the ACM Digital Library.

% TODO: move to correct place
\lstset{
  literate={©}{{\copyright}}1
}

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=AGIT Journal: Table of Contents A]
doc("http://dl.acm.org/results.cfm?query=%2A&filtered=acmPubGroups%2EacmPubGroup%3DDoctoral%20Dissertation&within=owners%2Eowner%3DGUIDE&dte=&bfr=&srt=publicationDate")
/(//*[@class="pagelogic"][1]/span[./strong]/following-sibling::span[./a][1]/{click[wait=2] /})*
  //*[@id='results']/div[contains(@class, 'details')]:<record>
    [? .//div[@class='title']//a:<title=normalize-space(.)>]
    [? .//div[@class='authors']//a:<author=normalize-space(.)>]
    [? .//div[@class='source']//span[@class='publicationDate']
      :<year=replace(normalize-space(.), ".*?(\d{4}).*", "$1")>
    ]
    [? .//div[@class='title']//a:<url=qualify-url(@href)>]
    [? .//div[@class='title']//a/{click[wait=2] /}/.
      [? .//*[@id='divmain']//span[contains(., '©')]/ancestor::td[1]
        :<affiliation=normalize-space(substring-before(., '©'))>]
      [? .//table[contains(., 'Title')]
        [? .//tr[contains(., 'Pages')]/td[2]:<pages=normalize-space(.)>]
        [? .//tr[contains(., 'ISBN')]/td[2]:<isbn=normalize-space(.)>]
      ]
      [.//a[contains(@href, 'preflayout=flat')]/{click /}
        //table[contains(., 'Title')]
          [? .//tr[contains(., 'Pages')]/td[2]:<pages=normalize-space(.)>]
          [? .//tr[contains(., 'ISBN')]/td[2]:<isbn=normalize-space(.)>]
      ]
    ]
\end{lstlisting}

%-------------------------------------------------------------------------
\subsection{Academic Content Platforms for Journals}
%-------------------------------------------------------------------------

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{Cambridge Core}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
The dblp crawling architecture leverages the evaluation of these OXPath expressions to extract records for Volume 26 of the Journal of Functional Programming in Cambridge Core\footnote{\url{https://www.cambridge.org/core}}.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Cambridge Core: List of Issues]
doc('https://www.cambridge.org/core/journals /journal-of-functional-programming/all-issues')
  //*[contains(@href, 'panel26')]:<volume>
    [ ./following-sibling::*//a:<issue>
      [ .:<url=qualify-url(@href)>]
      [? .[contains(. , 'Issue')] :<iss-number=replace(normalize-space(.), ".*?Issue.*?(\d+(-\d+)?|[A-Z]{1}).*", "$1")>]
      [? ./preceding::*[contains(@href, 'panel')][1]:<vol-number=replace(., ".*?Volume.*?(\d+(-\d+)?).*", "$1")>]
      [? ./following::*[@class="date"][1]
        :<year=replace(., ".*?(\w+).*?(\d{4}).*", "$2")>
        :<month=replace(., ".*?(\w+).*?(\d{4}).*", "$1")>] ]
\end{lstlisting}

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Cambridge Core: Table of Contents]
doc('https://www.cambridge.org/core/journals /journal-of-functional-programming/issue /125E787C7C2F92F68C6FC88EBD1A16F0')
  /?!(!?//hr[1]//following::*[@class='pagination'][1] //a[contains(., 'Next')]/{clkwithchange /}?!)*!?
  //div[@data-prod-id]:<article>
    [? .//li[@class="title"]
      [? ./a[@class="part-link"] :<title=normalize-space(.)>] ]
    [? .//li[@class="author"] :<authors=normalize-space(string-join( ./a[@class="more-by-this-author"], ', '))>]
    [? .//li[@class="source"]/a :<ee=normalize-space(.)>]
    [? .//li[@class="published"]
      [? .//*[@class="date"] :<date=normalize-space(.)>]
      [? .//following-sibling::*[@class="pages"] :<pages=replace(normalize-space(.), ".*?(\w?\d+(-\w?\d+)?)", "$1")>] ]
    [? .//preceding::h4[1] :<section=normalize-space(.)>]
\end{lstlisting}
%     [? .//preceding::*[@class="volume"]
%       [? .:<volume=replace(normalize-space(.), ".*?(\d+(-\d+)?)(.*?Issue.*?(\d+(-\d+)?))?.*", "$1")>]
%       [? .:<issue=replace(normalize-space(.), ".*?(\d+(-\d+)?)(.*?Issue.*?(\d+(-\d+)?))?.*", "$4")>] ]
%     [? .//preceding::*[@class="issue-date"]
%       [? .:<month=replace(normalize-space(.), ".*?(\w+).*?(\d{4}).*", "$1")>]
%       [? .:<year=replace(normalize-space(.), ".*?(\w+).*?(\d{4}).*", "$2")>] ]

\noindent By evaluating the OXPath expression in Listing 2 with an XML output handler, an XML document of the following structure is produced.
\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=xml,
caption=Cambridge Core: Example of XML output]
<?xml version="1.1" encoding="UTF-8"?>
<results><!--[...]-->
  <article>
    <title>Linear lambda terms as ...</title>
    <authors>NOAM ZEILBERGER</authors>
    <ee>https://doi.org/10.1017/...</ee>
    <date>04 November 2016</date>
    <pages>e21</pages>
    <section>Theoretical Pearls</section>
  </article>
  <!--[...]-->
</results>
\end{lstlisting}

% %-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
% \subsection{Oxford Academic}
% %-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

% The dblp crawling architecture leverages the evaluation of these OXPath expressions to extract records for Volume 26 of the Journal of Functional Programming in Cambridge Core\footnote{\url{https://www.cambridge.org/core}}.
%
% \begin{lstlisting}[%
% firstnumber=1,
% linewidth=\columnwidth,
% language=oxpath]
% doc('https://www.aclweb.org/anthology/K/K16/')
%   //*[@id='content']//p:<record>
%     [./a:<pdf=string(@href)>]
%     [./b:<authors=normalize-space(.)>]
%     [./i:<title=string(.)>]
%     [? ./preceding::h1[1]:<section=string(.)>]
% \end{lstlisting}

% \begin{lstlisting}[%
% firstnumber=1,
% linewidth=\columnwidth,
% language=oxpath]
% doc('https://www.aclweb.org/anthology/K/K16/')
%   //*[@id='content']//p:<record>
%     [./a:<pdf=string(@href)>]
%     [./b:<authors=normalize-space(.)>]
%     [./i:<title=string(.)>]
%     [? ./preceding::h1[1]:<section=string(.)>]
% \end{lstlisting}

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{Taylor \& Francis Online}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

The dblp crawling architecture leverages the evaluation of these OXPath expressions to extract records for Volume 9, Issue 6 of the International Journal of Computational Intelligence Systems in Taylor \& Francis Online\footnote{\url{http://www.tandfonline.com}}.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Taylor \& Francis Online: List of Issues]
doc('http://www.tandfonline.com/loi/tcis20')
  /.[? .//a[@class='btn']/{click /}]
  //ul[@class='list-of-issues'] //li[contains(@id, 'vol_9')][1]/a:<volume>
  [ ./{mouseover}/{click}
    /..//li[not(./img[contains(@alt, 'Progress')])]:<issue>
      [? ./ancestor::li:<vol-number=replace( normalize-space(.), ".*?Volume.*?(\d+(-\d+)?).*", "$1")>]
      [? ./a/div:<iss-number=replace(., ".*?Issue.*?(\d+(-\d+)?).*", "$1")>]
      [? .//*[@id='loiIssueCoverDateText'] :<year=normalize-space(.)>]
      [? ./a:<url=qualify-url(replace(@href, "(.*)\?.*", "$1"))>] ]
\end{lstlisting}

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Taylor \& Francis Online: Table of Contents]
doc('http://www.tandfonline.com/toc/tcis20/9/6')
  /.[? .//a[@class='btn']/{click /}]
  //*[@class="tocArticleEntry"]:<article>
    [? .//*[contains(@class, 'title')] :<title=normalize-space(.)>]
    [? .//*[contains(@class, 'type')] :<type=normalize-space(.)>]
    [? .//*[@class="articleEntryAuthorsLinks"] :<authors=normalize-space(string-join(./span, ', '))>]
    [? ./preceding::*[@class="tocHeading"][1] :<section=normalize-space(.)>]
    [? .//*[contains(@class, 'title')]/a :<ee=normalize-space(@href)>]
    [? .//*[contains(@class, 'tocPageRange')] :<pages=substring-after(., ': ')>]
\end{lstlisting}

%-------------------------------------------------------------------------
\subsection{Other Journal Publishers}
%-------------------------------------------------------------------------

The dblp crawling architecture leverages the evaluation of this OXPath expressions to extract records for the
\emph{AGIT Journal für Angewandte Geoinformatik}\footnote{\url{http://gispoint.de/agit-journal.html}}.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=AGIT Journal: List of Issues]
doc('http://gispoint.de/agit-journal.html')
  //*[contains(@class, 'listview ')]//*[@class='linktosingle']:<record>
    :<toc=qualify-url(@href)>
    :<volume=replace(., ".*?(\d+)\-(\d{4}).*", "$2")>
    :<issue=replace(., ".*?(\d+)\-(\d{4}).*", "$1")>
\end{lstlisting}

The following expression for the table of contents only extracts the URL to the detail page.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=AGIT Journal: Table of Contents A]
doc('http://gispoint.de/liste-artikel/agit.html ?tx_browser_pi1%5BIDedition%5D=1')
  //*[@class='item']:<record>
    [? ./*[contains(@class, 'author')]:<authors=normalize-space(.)>]
    [? ./*[contains(@class, 'title')]:<title=normalize-space(.)>
      /a:<details=qualify-url(@href)>
    ]
    [? .//*[@title][contains(., 'Open Access')]:<open-access>]
    [? ./*[contains(@class, 'pageBegin')]:<pages=normalize-space(.)>]
    [? ./*[contains(@class, 'doi')]:<doi=normalize-space(.)>]
    [? ./preceding::h2[1]:<section=normalize-space(.)>]
\end{lstlisting}

This expression for the table of contents follows the URL to the detail page for each article and also extracts the URL to the PDF file for each article.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=AGIT Journal: Table of Contents B]
doc('http://gispoint.de/liste-artikel/agit.html ?tx_browser_pi1%5BIDedition%5D=1')
  //*[@class='item']:<record>
    [? ./*[contains(@class, 'author')]:<authors=normalize-space(.)>]
    [? ./*[contains(@class, 'title')]:<title=normalize-space(.)>
      /a/{click /}//*[contains(@class, 'pdf_link')]/a:<pdf=qualify-url(@href)>
    ]
    [? .//*[@title][contains(., 'Open Access')]:<open-access>]
    [? ./*[contains(@class, 'pageBegin')]:<pages=normalize-space(.)>]
    [? ./*[contains(@class, 'doi')]:<ee=normalize-space(.)>]
    [? ./preceding::h2[1]:<section=normalize-space(.)>]
\end{lstlisting}

%-------------------------------------------------------------------------
\subsection{Conference Proceedings}
%-------------------------------------------------------------------------

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{ACL Anthology}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

The dblp crawling architecture leverages the evaluation of this OXPath expression to extract records for the Proceedings of the 20th SIGNLL Conference on Computational Natural Language Learning in the ACL Anthology\footnote{\url{http://aclweb.org/anthology}}.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=ACL Anthology: Table of Contents]
doc('https://www.aclweb.org/anthology/K/K16/')
  //*[@id='content']//p:<article>
    [ ./a:<pdf=string(@href)>]
    [ ./b:<authors=normalize-space(.)>]
    [ ./i:<title=string(.)>]
    [? ./preceding::h1[1]:<section=string(.)>]
\end{lstlisting}

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{Proceedings of SPIE}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

The dblp crawling architecture leverages the evaluation of this OXPath expression to extract records for \emph{Image Processing: Algorithms and Systems XIII} in the Proceedings of SPIE\footnote{\url{https://www.cambridge.org/core}}, Volume 9399.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Proceedings of SPIE: Table of Contents]
doc('http://proceedings.spiedigitallibrary.org /volume.aspx?volume=9399')
  //*[@class='articleContent']:<article>
    [? .//*[@class='articleTitle'] :<title=normalize-space(.)>]
    [? .//*[@class='authors'] :<authors=normalize-space(.)>]
    [? .//*[@class='doi'] :<ee=concat('http://dx.doi.org/', substring-after(., ': '))>]
    [? .//*[@class='articleInfo'] :<pages=replace(., ".*?([A-Z\d]+) \((.*)\).*", "$1")>
    :<date=replace(., ".*?([A-Z\d]+) \((.*)\).*", "$2")>]
    [? ./preceding::h2[1]:<section=string(.)>]
\end{lstlisting}
%     [? ./preceding::*[@class='pageHeader']/h1
%       /span[1]:<volume=substring-after(., 'Volume ')>
%       /following-sibling::span:<series=string(.)>/
%         ../following-sibling::*[@class='citation']/
%           *[@class='authors']:<editors=normalize-space(.)>/
%           ../text()[2]/
%             .:<place=replace(normalize-space(.),  "(.*?) \| (\w+).*?(\d+).*?(\d+)$", "$1")>/
%             .:<month=replace(normalize-space(.),  "(.*?) \| (\w+).*?(\d+).*?(\d+)$", "$2")>/
%             .:<start-day=replace(normalize-space(.),  "(.*?) \| (\w+).*?(\d+).*?(\d+)$", "$3")>/
%             .:<year=replace(normalize-space(.),  "(.*?) \| (\w+).*?(\d+).*?(\d+)$", "$4")>
%       ]

%-------------------------------------------------------------------------
\subsection{Digital Libraries}
%-------------------------------------------------------------------------

%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -
\subsubsection{Frontiers}
%-  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -  -

The dblp crawling architecture leverages the evaluation of these OXPath expressions to extract records for the published articles in a Frontiers\footnote{\url{http://journal.frontiersin.org}} journal archive. The required parameters are:
1)~Frontiers journal archive URL (\texttt{\$\{url\}}\footnote{e.g., \url{http://journal.frontiersin.org/journal/robotics-and-ai\#archive}}),
2)~a date range (\texttt{\$\{start.month\}}, e.g., 01, \texttt{\$\{start.day\}}, e.g., 01, \dots, \texttt{\$\{end.year\}}, e.g., 2016). The templates are evaluated sequentially in the same browser window with the same URL. By filling and submitting a date picker form, the first resolved template queries the backend database of Frontiers for all articles belonging to the date range in the specified journal archive and extracts their total count. That number is divided by 30 (number of articles loaded by scrolling to the end of the result list if there are more), rounded up, and used to resolve the variable \texttt{\$\{times\}} for the scroller template. Finally, the extractor crawls the result list of articles for published works only.

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Frontiers: Date Picker and Article Counter]
doc('${url}')
  //button[contains(@class,"filter-calender")] /{click}
  //following::input[contains(@name, "start")] /{"${start.month}/${start.day}/${start.year}"}
  /following::input[contains(@name,"end")] /{"${end.month}/${end.day}/${end.year}"} /{pressenter}
  /following::button[contains(@class,"applyBtn")] /{click/}
  //*[@*[contains(., "article-sorting")]]
    //*[@*[contains(., "title-number")]] :<count=string(.)>
\end{lstlisting}

\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Frontiers: Scroller]
doc('${url}')
  /(//*[contains(@class, "container-grid-box")] [last()]/{mouseover /}?!)*{0,${times}}!?
\end{lstlisting}
\newpage
\begin{lstlisting}[%
firstnumber=1,
linewidth=\columnwidth,
language=oxpath,
caption=Frontiers: Extractor]
doc('${url}')
  //*[contains(@class, "container-grid-box")]
    [ .//*[contains(@class, "teaser-meta") and
      contains(string(.), "Published on")]]
    /.:<record>
      [? .//*[contains(@class, "-heading")] :<title=normalize-space(.)>]
      [? .//*[contains(@class, "teaser-authors")] :<authors=normalize-space(.)>]
      [? .//*[contains(@class, "teaser-meta")] :<ee=concat('http://dx.doi.org/', normalize-space(substring-after(., "doi: ")))>/strong:<date=substring-after(., "Published on ")>]
\end{lstlisting}

%------------------------------------------------------------------------------
% \section{Crawling}\label{oia:crawling}
%------------------------------------------------------------------------------
%
% \begin{example}
%
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/tandf_loi-0.png}
% 	\caption{Computer science journals on DBLP website\label{fig:oia:crawling:tandf_loi:0}}
% \end{figure}
%
% ...
%
% \begin{lstlisting}[language=OXPath]
% doc('${url}', [wait=5])
%   //ul[@class='list-of-issues']//li[contains(@id, 'vol_${volume}')]/a/{click[wait=1]}
%     /..//li[not(./img[contains(@alt, 'Progress')])]:<record>
%       [? ./ancestor::li:<volume=replace(normalize-space(.), "Volume (\d+(-\d+)?).*", "$1")>]
%       [? ./a/div:<issue=replace(normalize-space(.), "Issue (\d+(-\d+)?).*", "$1")>]
%       [? .//*[@id='loiIssueCoverDateText'] :<year=normalize-space(.)>]
%       [? ./a:<url=concat('http://www.tandfonline.com', replace(normalize-space(@href), "(.*)\?.*", "$1"))>]
% \end{lstlisting}
%
% \end{example}
%
% TODO:
%
% \begin{itemize}
%   \item lists of issues inaccessible:
%   \begin{itemize}
%     \item solutions:
%     \begin{itemize}
%       \item modify url
%       \item {4.2} or here: click volume before accessing issues
%     \end{itemize}
%   \end{itemize}
% \end{itemize}
%
% %------------------------------------------------------------------------------
% \section{Interaction}\label{oia:interaction}
% %------------------------------------------------------------------------------
%
% \begin{example}
%
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=12cm]{users/chapters/graphics/oxpathInAction/tandf_toc-0.png}
% 	\caption{Computer science journals on DBLP website\label{fig:oia:crawling:tandf_toc:0}}
% \end{figure}
%
% ...
%
% \begin{lstlisting}[language=OXPath]
% doc('${url}')
%   //a[@class='btn']/{click /}
%     //*[@class="tocArticleEntry"][.//*[contains(@class, 'title')]]:<record>
%       [.//*[contains(@class, 'title')]:<title=replace(normalize-space(.), "<", "&lt;")>]
%       [? .//*[contains(@class, 'type')]:<type=normalize-space(.)>]
%       [? .//*[@class="articleEntryAuthorsLinks"]:<authors=normalize-space(string-join(./span, ', '))>]
%       [? .//preceding::h3[./span[@class="special"]]:<header=normalize-space(.)>]
%       [? .//preceding::h3:<header=normalize-space(.)>]
%       [? .//preceding::*[@class="tocHeading"][1]:<section=normalize-space(.)>]
%       [? .//preceding::*[@id='tocList']//a[contains(@class, 'open')]//span[@class="slider-vol-no"]:<volume=replace(normalize-space(.), "Volume (\d{1,2}),", "$1")>]
%       [? .//preceding::*[@id='tocList']//a[@class='open']/span:<issue=normalize-space(.)>]
%       [? .//preceding::*[@id='tocList']//a[contains(@class, 'open')]//span[@class="slider-vol-year"]:<year=normalize-space(.)>]
%       [? .//*[contains(@class, 'title')]/a:<ee-fallback=concat('http://www.tandfonline.com', normalize-space(@href))>]
%       [? .//*[contains(@class, 'title')]/a/{click[wait=2] /}
%         /.[? .//*[@class="itemPageRangeHistory"]:<pages=normalize-space(substring-after(substring-before(., '|'), ' '))>]
%           [? .//*[@class='dx-doi']/a:<ee=normalize-space(.)>]
%           [? .//p/a[contains(@href, 'http://dx.doi.org/')]:<url=normalize-space(.)>]
%       ]
% \end{lstlisting}
%
% \end{example}
%
% TODO:
%
% \begin{itemize}
%   \item accept use of cookies to get rid of overlay (click)
%   \item access abstract page for additional information (click)
% \end{itemize}
%
% %------------------------------------------------------------------------------
% \section{Extraction}\label{oia:extraction}
% %------------------------------------------------------------------------------
%
% TODO:
%
% \begin{itemize}
%   \item extracting from list
%   \item including optional/fallback information
%   \item axis: preceding for common information
% \end{itemize}
%
% %------------------------------------------------------------------------------
% \section{Problems}\label{oia:problems}
% %------------------------------------------------------------------------------
%
% TODO:
%
% \begin{itemize}
%   \item order of attribute markers: non-optionals first
%   \item ...
% \end{itemize}


==> users/chapters/postprocessing.tex <==
%-------------------------------------------------------------------------------
\chapter{Post-Processing}
%-------------------------------------------------------------------------------

